A Review of the Role of Causality in Developing Trustworthy AI Systems

State-of-the-art AI models largely lack an understanding of the cause-effect relationship that governs human understanding of the real world. Consequently, these models do not generalize to unseen data, often produce unfair results, and are difficult to interpret. This has led to efforts to improve the trustworthiness aspects of AI models. Recently, causal modeling and inference methods have emerged as powerful tools. This review aims to provide the reader with an overview of causal methods that have been developed to improve the trustworthiness of AI models. We hope that our contribution will motivate future research on causality-based solutions for trustworthy AI.

==> 7B_appl_social.tex <==
\iffalse
\subsection{Causality in Social Media and Online Platforms}

\subsubsection{Causal models for recommendations}
Causal Disentanglement with Network Information for Debiased Recommendations~\cite{sheth2022causal}

Causal Intervention for Leveraging Popularity Bias in Recommendation [SIGIR 21]

\subsubsection{Causal models for detecting fake news}
%\gourab{I would prefer some other general application domain than having this very specific domain with limited works.}
Domain Adaptive Fake News Detection via Reinforcement Learning~\cite{mosallanezhad2022domain}

Generalizing to the Future: Mitigating Entity Bias in Fake News Detection [SIGIR 22]

Bias Mitigation for Evidence-aware Fake News Detection by Causal Intervention [SIGIR 22]

Causality and Uncertainty of Information for Content Understanding~\cite{raglin2020causality}
\fi

\subsection{Causality in Online Social Media}

 A growing body of work has hence concentrated on deploying causal methods in analyzing social media data and correcting for such biases, which we discuss in this section. 
Broadly, we segregate the papers into two categories - (i) \textbf{impact analysis} and (ii) \textbf{decision making}.  

\begin{figure} 
  \centering   
    \begin{forest}
      for tree={
%        minimum height=0.75cm,
%        if level=0
%            {fill=gray,
%            text=white}
%            {fill=lightgray},
%        rounded corners=4pt,
        parent anchor=south,
        child anchor=north,
        fit=band,
      }
      [Causality in online social media
        %[Differential Privacy \\\cite{tschantz2020sok}
        %]
        %[Federated learning
          [\textbf{Impact analysis}
          [Feature selection]
          [Removing bias]
          [Domain adoptation]
          ]
          [\textbf{Decision making}
          [Online Ads]
          [Retrieval and ranking]
          [Recommender systems]
          ]
        %]
      ]
    \end{forest}
    \caption{Causality and privacy approaches.}
    \label{fig:fairness_tree}
\end{figure}

\iffalse
\subsubsection{\bf Impact analysis}: The key objective of this category of papers is to analyze the impact of a particular treatment on an outcome. For example, in \cite{verma2022examining}, the authors examine the impact of sharing misinformation about Covid-19 on social media on a person's mental health. In this case, the treatment is sharing misinformation while the outcome is a person's anxiety level. The general methodology deployed in this category of papers is the PO framework on observed data. The population is divided into treated and untreated groups and the difference in average outcome quantifies the effect/impact of the treatment. In the covid-19/misinformation example, the users sharing misinformation are considered as the treatment group while those not sharing the information as the untreated group. To ensure that the individuals belonging to the treated and untreated groups are similar on average (in terms of a pre-defined set of characteristics/covariates), matching~\cite{imbens2015causal} is deployed. Depending on their application area, we further classify the papers in this category into - (i) mental health, (ii) opinion dynamics and (iii) platform <will have to come up with a better name>.

\paragraph{Mental health}: Millions of individuals share personal experiences and opinions on online social media platforms. This allows for unobtrusive, self-reported data of the emotional state of individuals, which could be utilized to perform large scale analysis of mental health of individuals. In \cite{de2016discovering}, the authors utilize reddit\footnote{https://www.reddit.com/} data to understand shifts to suicidal ideation. The individuals are differentiated based on whether they post only on the mental health (MH) subreddits or transition from posting on MH to posting on suicide watch (SW) subreddits. Stratified propensity score based matching is deployed to match individuals in the two groups and the outcome is measured in terms of linguistic structure, interpersonal awareness and interaction. For example, the individuals transitioning to SW show lower social engagement, often writing longer and fewer posts. In a follow-up work~\cite{de2017language}, deploying a similar dataset and methodology, the authors analyze how the language of comments in
Reddit mental health communities influences risk to suicidal ideation in the future. 
\fi

\subsubsection{\bf Impact analysis}: Its ubiquitous nature and wide-spread use, makes online social media a unique platform for understanding human behavior on a massive scale. The data collected from online social media are also often used in training large scale machine learning models on tasks such as sentiment classification, fake news detection, recommendation among others. However, existing research have demonstrated that social media data often consists of unwanted biases, which when used as training data can have negative impact on the trained model. Hence, a growing body of research has been dedicated towards adopting causal methods as an aid in training machine learning models through - (i) feature selection, (ii) removing selection bias and (iii) domain adaptation.

\paragraph{\bf Feature selection:} Data collected from online social media are unstructured. Hence, the practitioners often resort to devising hand-crafted features when building a machine learning model. However, it is unclear which features should be considered while training the model. In the existing literature, the PO framework has often been deployed to understand causal relationships between the features and the outcome. Such an analysis can help in identifying important features and thereby help in building a model that is robust and interpretable. A particular use-case where such analysis has often been deployed is analyzing mental health issues from social media post~\cite{de2013predicting}. In \cite{de2016discovering}, the authors identify linguistic structure, interpersonal awareness, interaction as distinct markers for predicting shifts to suicide ideation. \cite{mitchell2015quantifying, mcmanus2015mining} identify linguistic markers to detecting  individuals suffering from schizophrenia. Utilizing these makers in designing classifiers not only leads to better performance, but also aids in improving the robustness and interpretability of the model. 

\paragraph{\bf Detecting and removing bias:} Online social media is also utilized as a source for obtaining large scale training dataset for training machine learning models on tasks such as fake news and hate speech detection among others. Recent works have demonstrated that these datasets often contain hidden biases which can have a negative impact on the models trained on them. Getting rid of such biases could help in training more robust models.  In~\cite{zhou2021hidden}, the authors observe that models trained on  FakeNewsnet dataset~\cite{shu2017fake} consider celebrity names as a distinguishing feature for classifying a news article as fake. The author relate this behavior to the selection bias as most fake news articles contain a click-bait title mentioning celebrities while it is not so for reliable news articles. \cite{arango2019hate} notes similar biases in hate speech detection datasets as the users sharing hate speech account for a very small portion of the entire user population. 
\cite{wu2022bias} proposes to get rid of such biases in fake news detection through causal intervention. In this framework, the model is first trained on the original biased dataset and during test phase it makes predictions simultaneously on the conventional and counterfactual predictions (obtained based on intervened evidence). Unbiased predictions are obtained by subtracting intervened outputs from the conventional ones. 
\cite{cheng2021causal} considers the problem of fake news dissemination and proposes a systematic approach drawing on causal methods that alleviates selection bias. \cite{zhu2022generalizing} points out presence of entity bias in fake news datasets and its effect over time. For example, the entity ``Donald Trump'' is encountered more frequently in  News articles published in 2010-2017 while it reduces significantly in 2018. Based on a causal graph among entities, news contents, and news veracity, the authors propose to  separately model the contribution of each cause (entities and
contents) during training. The direct effect of entities is then removed during inference. Similar methods are adopted for mitigating bias in text classification~\cite{qian2021counterfactual}. 

\paragraph{\bf Domain adaptation:}
